Anti-Adversarially Manipulated Attributions for Weakly and Semi-Supervised Semantic Segmentation

Weakly supervised semantic segmentation produces a pixel-level localization from a classifier, but it is likely to restrict its focus to a small discriminative region of the target object. AdvCAM is an attribution map of an image that is manipulated to increase the classification score. This manipulation is realized in an anti-adversarial manner, which perturbs the images along pixel gradients in the opposite direction from those used in an adversarial attack. It forces regions initially considered not to be discriminative to become involved in subsequent classifications, and produces attribution maps that successively identify more regions of the target object. In addition, we introduce a new regularization procedure that inhibits the incorrect attribution of regions unrelated to the target object and limits the attributions of the regions that already have high scores. On PASCAL VOC 2012 test images, we achieve mIoUs of 68.0 and 76.9 for weakly and semi-supervised semantic segmentation respectively, which represent a new state-of-the-art.

==> latex/Figures/suppressing_reg.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{latex/Figures/suppressing_examples_v3.pdf}
\caption{\label{appendix_eachiter_ex_realex} Examples of initial CAMs and successive localization maps obtained from images manipulated by iterative adversarial climbing.}
% Effectiveness of regularization technique. (\textit{Left}) Seed quality on mIoU (\%). (\textit{Right}) 1-precision (\%)}
\end{figure*}

